On the possible mechanism of radio emission of polars

We suggest a mechanism for generation of radio emission from polars. It is based on the cyclotron radiation of thermal electrons at the background of fluctuating magnetic field. The source of fluctuations is Alfv\'{e}n wave turbulence. Expressions for the radiation spectrum and degree of polarization are obtained. By the example of the polar AM~Her, the fluxes of radio emission from the accretion stream are calculated. Within the framework of proposed emission model, with realistic plasma characteristics, it is possible to reproduce observed radiation fluxes in the VLA bands.

==> Makefile <==

OUT := kurbatov_etal_radio_emission
TARGET := radio_emission


$(TARGET).ps: $(TARGET).dvi
	dvips $(TARGET)

$(TARGET).dvi: $(TARGET).tex $(TARGET).bbl
	latex $(TARGET)
	latex $(TARGET)

.PHONY: bib bbl
bib bbl: $(TARGET).bbl

$(TARGET).bbl: $(TARGET).bib
	latex $(TARGET)
	bibtex $(TARGET)

.PHONY: pdf
pdf: $(OUT).pdf

$(OUT).pdf: $(TARGET).ps
	ps2pdf $(TARGET).ps $@


.PHONY: zip
zip:
	zip $(OUT).zip Makefile *.eps *.tex *.bib *.sty


.PHONY: clean
clean:
	rm -f *.log *~ $(OUT).pdf $(OUT).zip \
		$(addprefix $(TARGET),.dvi .ps .pdf .aux .log .bbl .blg .out)

